Detecting and Understanding Real-World Differential Performance Bugs in Machine Learning Libraries

Programming errors that degrade the performance of systems are widespread, yet there is little tool support for analyzing these bugs. We present a method based on differential performance analysis---we find inputs for which the performance varies widely, despite having the same size. To ensure that the differences in the performance are robust (i.e. hold also for large inputs), we compare the performance of not only single inputs, but of classes of inputs, where each class has similar inputs parameterized by their size. Thus, each class is represented by a performance function from the input size to performance. Importantly, we also provide an explanation for why the performance differs in a form that can be readily used to fix a performance bug. The two main phases in our method are discovery with fuzzing and explanation with decision tree classifiers, each of which is supported by clustering. First, we propose an evolutionary fuzzing algorithm to generate inputs. For this fuzzing task, the unique challenge is that we not only need the input class with the worst performance, but rather a set of classes exhibiting differential performance. We use clustering to merge similar input classes which significantly improves the efficiency of our fuzzer. Second, we explain the differential performance in terms of program inputs and internals. We adapt discriminant learning approaches with clustering and decision trees to localize suspicious code regions. We applied our techniques to a set of applications. On a set of micro-benchmarks, we show that our approach outperforms state-of-the-art fuzzers in finding inputs to characterize the differential performance. On a set of case-studies, we discover and explain multiple performance bugs in popular machine learning frameworks. Four of these bugs, reported first in this paper, have since been fixed by the developers.

==> Makefile <==
# NOTE: you must install latexmk first!!

LATEX=pdflatex
LATEXOPT=--shell-escape
NONSTOP=--interaction=nonstopmode

LATEXMK=latexmk
LATEXMKOPT=-pdf
CONTINUOUS=-pvc

MAIN=main
SOURCES=$(MAIN).tex Makefile overview.tex header.tex introduction.tex overview.tex definition.tex approach.tex experiment.tex case-study.tex related.tex papers.bib implementations.tex papers.bib related.tex conclusion.tex Threat-to-validity.tex ack.tex
FIGURES=

all:    $(MAIN).pdf

.refresh:
	touch .refresh

$(MAIN).pdf: $(MAIN).tex .refresh $(SOURCES) $(FIGURES)
	$(LATEXMK) $(LATEXMKOPT) \
	-pdflatex="$(LATEX) $(LATEXOPT) %O %S" $(MAIN)

online: $(MAIN).tex .refresh $(SOURCES) $(FIGURES)
	$(LATEXMK) $(LATEXMKOPT) $(CONTINUOUS) \
	-pdflatex="$(LATEX) $(LATEXOPT) $(NONSTOP) %O %S" $(MAIN)

force:
	touch .refresh
	rm $(MAIN).pdf
	$(LATEXMK) $(LATEXMKOPT) \
		-pdflatex="$(LATEX) $(LATEXOPT) %O %S" $(MAIN)

clean:
	$(LATEXMK) -C $(MAIN)
	rm -f $(MAIN).pdfsync
	rm -rf *~ *.tmp
	rm -f *.bbl *.blg *.aux *.end *.fls *.log *.out *.fdb_latexmk *.refresh *.DS_Store

once:
	$(LATEXMK) $(LATEXMKOPT) -pdflatex="$(LATEX) $(LATEXOPT) %O %S" $(MAIN)

debug:
	$(LATEX) $(LATEXOPT) $(MAIN)

.PHONY: clean force once all

